Causal inference for data-driven debugging and decision making in cloud computing

Cloud computing involves complex technical and economical systems and interactions. This brings about various challenges, two of which are: (1) debugging and control to optimize the performance of computing systems, with the help of sandbox experiments, and (2) privacy-preserving prediction of the cost of ``spot'' resources for decision making of cloud clients. In this paper, we formalize debugging by counterfactual probabilities and control by post-(soft-)interventional probabilities. We prove that counterfactuals can approximately be calculated from a ``stochastic'' graphical causal model (while they are originally defined only for ``deterministic'' functional causal models), and based on this sketch a data-driven approach to address problem (1). To address problem (2), we formalize bidding by post-(soft-)interventional probabilities and present a simple mathematical result on approximate integration of ``incomplete'' conditional probability distributions. We show how this can be used by cloud clients to trade off privacy against predictability of the outcome of their bidding actions in a toy scenario. We report experiments on simulated and real data.

==> include/plot_exp1_resampling.tex <==
% This file was created by matplotlib2tikz v0.5.4.
% The lastest updates can be retrieved from
% 
% https://github.com/nschloe/matplotlib2tikz
% 
% where you can also submit bug reports and leavecomments.
% 
\begin{tikzpicture}

\begin{axis}[
xmin=7, xmax=15,
ymin=0, ymax=120000000,
axis on top,
width=\figurewidth,
height=\figureheight
]
\addplot [white!66.666666666666657!black, mark=x, mark size=3, only marks]
table {%
7 6966485
7 10172358
7 20967633
7 9337210
7 25989552
7 14068097
7 15362152
7 12515977
7 4773525
7 6780694
7 32456200
7 10683914
7 2040862
7 4759218
7 18471140
7 46398032
7 10516786
7 28485554
7 19051590
7 16695102
7 18980129
7 5061185
7 8296596
7 21740986
7 5516717
7 7277958
7 18310683
7 19159530
7 26387816
7 10955749
7 19432339
7 28153617
7 8653786
7 23383633
7 26078958
7 19203333
7 25177287
7 14808511
7 21347717
7 19714693
7 21231259
7 19827177
7 46879156
7 12358061
7 22007768
7 6180605
7 6710169
7 26684912
7 35989306
7 39855198
7 16847642
7 14665229
7 20357524
7 14675461
7 37564048
7 8776228
7 18570683
7 32183037
7 14697277
7 20778678
7 47238730
7 13857293
7 26295945
7 43534039
7 14566651
7 47391447
7 9349445
7 22086252
7 7520188
7 18320391
7 12973698
7 29219704
7 3561982
7 26711278
7 4338654
7 14988850
7 7445901
7 17862512
7 23195826
7 5123351
7 14639723
7 20424031
7 2027866
7 5963839
7 18343750
7 3555637
7 18314622
7 22141718
7 6541002
7 15458067
7 9131377
7 28141589
7 15306417
7 20737165
7 34546738
7 14211514
7 5698892
7 16111860
7 23624832
7 20904179
7 10980558
7 20851001
7 14941251
7 24174224
7 16115242
7 19450326
7 18320304
7 2986825
7 8692878
7 9416596
7 12280753
7 46279808
7 24911639
7 14363235
7 14646248
7 9679321
7 14808203
7 40741375
7 21957589
7 12894695
7 16496104
7 29998265
7 5547103
7 17549998
7 19260924
7 9664746
8 12780926
8 24905952
8 9822090
8 13581529
8 7566159
8 9248392
8 35643489
8 13125354
8 21151224
8 21547625
8 17362337
8 14764761
8 14445512
8 23560241
8 17147090
8 5700215
8 22564403
8 27402816
8 3459914
8 24552969
8 31263250
8 15047284
8 5665006
8 15836197
8 25245605
8 36510327
8 28766529
8 4749950
8 10799955
8 23167603
8 21186074
8 8760338
8 6873307
8 20375159
8 18476951
8 24832296
8 28162593
8 29709270
8 27993934
8 9620013
8 25469023
8 8825358
8 7544495
8 4386871
8 46800987
8 5560672
8 25075288
8 21387614
8 8274080
8 33962484
8 25627266
8 7877163
8 24292317
8 12502673
8 6805132
8 27882342
8 32717915
8 32020647
8 19246167
8 16613806
8 23155465
8 16280078
8 7025911
8 20354987
8 9709922
8 4520728
8 23120030
8 17941231
8 23536197
8 17441617
8 12769207
8 7207234
8 4450153
8 9924906
8 20484704
8 14870712
8 3814032
8 8518698
8 13442899
8 10565354
8 14330990
8 17164143
8 4500370
8 22220585
8 8902758
8 34904780
8 9395726
8 9333807
8 15233538
8 20290408
8 4701402
8 9035364
8 5959834
8 8610132
8 18993859
8 6228466
8 17860318
8 4351021
8 3736930
8 4530072
8 7267547
8 16782959
8 6213768
8 21137970
8 23685086
8 22325669
8 13846036
8 13708720
8 6709729
8 10069533
8 6410215
8 15556833
8 16579862
8 9366002
8 21272996
8 25039740
8 7188555
8 32173816
8 20667677
8 31574485
8 14254797
8 26968133
8 23903242
8 18041256
8 15992216
8 11488359
9 6332579
9 16994986
9 23557469
9 40530195
9 17916863
9 18212275
9 6036626
9 48362434
9 16671046
9 31934231
9 14033521
9 13224069
9 20622050
9 20675276
9 18728600
9 19631616
9 12755500
9 19220419
9 5961226
9 4268717
9 16595941
9 15901737
9 13196612
9 19065917
9 5405324
9 16969709
9 7363655
9 26447654
9 9360698
9 16772002
9 29511969
9 26381359
9 10701438
9 30239139
9 9846616
9 17718282
9 22440930
9 13981845
9 20984602
9 49542044
9 26939129
9 44643940
9 36508133
9 36843896
9 21640012
9 47380626
9 21845010
9 18991191
9 19754874
9 24586480
9 47106123
9 17479272
9 38450869
9 26297904
9 9435535
9 9737581
9 46183823
9 12384797
9 46969532
9 16410298
9 39653600
9 27409842
9 35204546
9 24426289
9 16479108
9 30635183
9 38471933
9 17348231
9 38421629
9 30318595
9 25568671
9 5727872
9 17808386
9 28921706
9 31419200
9 19444134
9 27380215
9 20749098
9 24468449
9 8598479
9 17108901
9 46349138
9 9715519
9 47238842
9 47681111
9 22468545
9 22582361
9 22142642
9 14425915
9 14929075
9 14500438
9 14278753
9 39713082
9 31112574
9 26256048
9 24080492
9 14837953
9 23306927
9 24586303
9 47291372
9 8899760
9 5665896
9 20447535
9 7192483
9 35279915
9 21935326
9 29220232
9 24626149
9 6308780
9 10373666
9 18963942
9 12671177
9 34936006
9 10765959
9 47396210
9 5069497
9 35653210
9 34454252
9 26824543
9 20752031
9 20768922
9 5320042
9 5717081
9 31650130
9 42862230
9 10823869
9 31817398
9 17188653
10 14002382
10 19478223
10 15743513
10 20332450
10 5946374
10 13547964
10 12958979
10 31506857
10 7036809
10 5604805
10 18432816
10 26005990
10 42766183
10 5674899
10 47701438
10 5382650
10 6397747
10 8619873
10 20337526
10 70619971
10 20650367
10 21322494
10 21558664
10 11455484
10 20994223
10 27686055
10 17400801
10 16033732
10 7336898
10 10020651
10 20947048
10 16831422
10 33432392
10 34135795
10 23178193
10 11114777
10 15359973
10 7717998
10 24295165
10 16389457
10 21229247
10 10282483
10 47909029
10 32907878
10 55435628
10 17350508
10 7474106
10 12494139
10 33364061
10 19262916
10 23391363
10 27836149
10 28520566
10 29566554
10 34010948
10 20241034
10 25515247
10 27564979
10 47162080
10 11294685
10 20474467
10 22818674
10 34931976
10 43382965
10 47820764
10 25769120
10 33892784
10 11610296
10 35848661
10 14091853
10 12226280
10 20051197
10 9274418
10 17919416
10 11651410
10 20573039
10 56495024
10 12227009
10 10282043
10 78357712
10 16211907
10 14393624
10 10413858
10 23720449
10 37485988
10 7198728
10 23928194
10 29528108
10 17422610
10 17150827
10 11343313
10 28476037
10 35818046
10 17115355
10 11425735
10 27025673
10 20803997
10 27812105
10 8982862
10 22392034
10 45401614
10 13588388
10 21018102
10 47581268
10 7225286
10 16615899
10 19186191
10 25041061
10 46748841
10 22011588
10 22416827
10 8707826
10 27567574
10 18474881
10 10491045
10 47581661
10 15962030
10 11414746
10 22824200
10 15385739
10 31671899
10 22169493
10 35155088
10 19890738
10 8587452
10 46959570
10 15729621
10 13071288
10 5239458
10 15232730
10 46022592
11 8580177
11 30895673
11 5750775
11 11919188
11 46910226
11 30355895
11 11504161
11 27107292
11 24408137
11 21331112
11 81783810
11 25135267
11 23963123
11 22288045
11 10480651
11 44492975
11 6881096
11 8316616
11 9218062
11 22402924
11 18799317
11 41287479
11 35276934
11 8514848
11 18279918
11 11602269
11 47154359
11 20423173
11 47818286
11 21614377
11 20585367
11 19914401
11 34866981
11 46128323
11 15270235
11 37613307
11 10325030
11 17328444
11 19817053
11 14478352
11 55289379
11 7326024
11 11791139
11 18966358
11 30345663
11 15054212
11 24356279
11 22932426
11 17117610
11 32645117
11 17392934
11 19819327
11 14063259
11 30699481
11 20436121
11 78999940
11 12679706
11 14146400
11 9494973
11 46216976
11 23474440
11 47471511
11 26547262
11 32996954
11 66452453
11 6441393
11 16955030
11 20089664
11 9920183
11 12125222
11 21135715
11 15023794
11 18829294
11 23898506
11 15874615
11 13918466
11 11064259
11 6910855
11 14379766
11 10663817
11 18849854
11 27206030
11 26914899
11 46904048
11 51888259
11 46772249
11 31109784
11 5948274
11 6464307
11 23534590
11 21639000
11 23057598
11 17648451
11 18496493
11 7591183
11 20866163
11 15362642
11 30687485
11 44447443
11 25412358
11 67884591
11 46546568
11 49403439
11 8208782
11 19307852
11 11926977
11 39229629
11 18584381
11 14339886
11 19891206
11 14207838
11 56495611
11 5649277
11 33591904
11 30957538
11 6930684
11 14194274
11 29094789
11 13088421
11 22824992
11 11496260
11 28089866
11 8294612
11 48017124
11 7651575
11 23214755
11 18834806
11 28151184
11 18260531
11 10490644
12 21456540
12 46510060
12 5809384
12 27021599
12 25059938
12 24938097
12 47173940
12 14717033
12 21446115
12 9650247
12 13909403
12 23570607
12 27479946
12 10121453
12 52968295
12 14313330
12 35386656
12 11463660
12 23440878
12 46927638
12 12019875
12 4088344
12 27604547
12 11851145
12 15166363
12 46881126
12 23737205
12 20611378
12 5995192
12 25171267
12 17797918
12 20070756
12 14252571
12 25774822
12 46907134
12 29052502
12 39816424
12 46504588
12 46844940
12 9367593
12 18289334
12 13614361
12 46843937
12 8137771
12 78862513
12 17951371
12 101406736
12 47351619
12 11411837
12 18582425
12 33825243
12 18599848
12 17229515
12 22842691
12 46808486
12 40531591
12 20588472
12 16277871
12 19770140
12 22569073
12 10745999
12 17691278
12 28165138
12 20720192
12 18619420
12 27405232
12 19517159
12 20151321
12 19302536
12 29855071
12 24867073
12 11476313
12 49374298
12 31983989
12 15541635
12 12148538
12 6369143
12 22884479
12 36223099
12 13637755
12 46347202
12 20373242
12 20859571
12 5939350
12 6716913
12 39153856
12 5875642
12 20607774
12 12668811
12 8231326
12 10747857
12 18802240
12 4909996
12 37722822
12 23505793
12 24383319
12 10188798
12 47200432
12 9763588
12 14069087
12 18610576
12 38804354
12 7789273
12 27533221
12 28162750
12 6832733
12 9097163
12 21659828
12 14109958
12 43877964
12 24508560
12 47437507
12 4666088
12 15244569
12 24136442
12 15479098
12 28051122
12 46236044
12 8317664
12 22961205
12 24962025
12 23329511
12 6520183
12 17172241
12 44554933
12 23540482
12 28277767
12 7684669
12 22439066
13 24095130
13 12225425
13 27551995
13 11580530
13 46205148
13 28897534
13 6443762
13 49350408
13 46926815
13 19199333
13 17657962
13 20782933
13 47799802
13 23008221
13 35350746
13 5122261
13 10948161
13 49969523
13 22390448
13 21412794
13 19465513
13 21697455
13 19343712
13 14768920
13 20236129
13 7615607
13 37742984
13 13365557
13 23213230
13 18127270
13 24786340
13 93548070
13 28353490
13 22491183
13 77028802
13 15725258
13 28012231
13 7884660
13 54667107
13 15069718
13 46741318
13 33357930
13 66341776
13 6880100
13 42581947
13 19513296
13 93269217
13 39343140
13 5335410
13 44210067
13 9379537
13 46475138
13 23357066
13 46881911
13 26193014
13 25988110
13 50139924
13 14936221
13 11082662
13 56615199
13 9915407
13 18174292
13 70818328
13 27674745
13 47522805
13 16733592
13 20667846
13 29872613
13 17150546
13 42411331
13 32076509
13 18725680
13 23255559
13 47224535
13 6537602
13 25828721
13 26468725
13 22673141
13 12640434
13 46453363
13 10117578
13 13838786
13 40575828
13 20234077
13 18903045
13 47014109
13 29799087
13 17827085
13 5950780
13 16337495
13 19343295
13 15882044
13 29180779
13 56170946
13 27304075
13 23473176
13 39505759
13 31182592
13 18633845
13 7657323
13 25359397
13 19271348
13 25975270
13 20922920
13 20909580
13 26454250
13 25348882
13 21821469
13 7700405
13 28985063
13 25785917
13 19866934
13 22767501
13 20980584
13 8397981
13 33652719
13 40722224
13 6243845
13 16790225
13 46654380
13 21121180
13 47535570
13 18069338
13 18893877
13 55386423
13 7187929
13 39340246
13 24392913
13 38692411
13 47365757
13 24404565
13 47272228
14 19518287
14 14874805
14 31468263
14 20266058
14 48030662
14 7330564
14 48407627
14 46203914
14 22315852
14 29607858
14 50557738
14 7831163
14 12508298
14 19271491
14 12118443
14 13549668
14 8466643
14 31832939
14 47379949
14 21215173
14 6102236
14 39951466
14 26245025
14 27150733
14 13993330
14 8940839
14 16155187
14 27131895
14 23516573
14 25225855
14 15435849
14 25344511
14 18747960
14 14242878
14 54165421
14 9786343
14 29363594
14 19538869
14 46739026
14 19877862
14 68968101
14 19778749
14 21596066
14 43976815
14 30356856
14 27156407
14 8985535
14 25976501
14 7357946
14 27677880
14 46542739
14 30119917
14 10387393
14 35825791
14 15988802
14 28791282
14 17500619
14 24152972
14 40536293
14 19459327
14 21603285
14 39777123
14 24415168
14 8904518
14 29314504
14 18491712
14 19071781
14 11648150
14 23169739
14 8693439
14 23252436
14 46209019
14 43890815
14 60460594
14 17667423
14 11785979
14 12211097
14 11610181
14 47663509
14 10149955
14 26752068
14 9309336
14 12150274
14 44758664
14 17253470
14 30915239
14 68470278
14 46584070
14 24332576
14 28525008
14 14686108
14 12609702
14 18018360
14 25220196
14 46715897
14 20628749
14 40979012
14 25086136
14 66245603
14 22024409
14 6891516
14 10687675
14 22563417
14 45525973
14 13394277
14 13228357
14 42108366
14 14809612
14 6956471
14 28646941
14 7426450
14 55628123
14 7894307
14 21025101
14 39287312
14 11737225
14 12968336
14 10846269
14 25026000
14 53343877
14 7204101
14 47262342
14 53656694
14 47253001
14 24314567
14 46996448
14 18882960
14 88383915
14 13748279
14 46090873
15 19664908
15 13987689
15 18724879
15 17927381
15 25245164
15 36119297
15 15826980
15 25896890
15 47662417
15 47589842
15 10927665
15 9522958
15 6907145
15 47297369
15 18002396
15 59887583
15 24939237
15 23910846
15 26567899
15 10264618
15 5892721
15 7379343
15 27172543
15 36145063
15 9630579
15 46710019
15 23351453
15 19021368
15 13105957
15 36454241
15 13891394
15 41245225
15 21063187
15 45713838
15 26751082
15 27696777
15 11302277
15 20990923
15 28105597
15 28181938
15 20737096
15 11088166
15 45018550
15 24570839
15 45053276
15 28305689
15 23160806
15 46018261
15 15336967
15 22129750
15 21825271
15 21475928
15 49721939
15 47513354
15 9719361
15 5621848
15 23492413
15 10504779
15 8778298
15 20361342
15 97190632
15 15952588
15 53756768
15 47186971
15 19106723
15 16992811
15 21360762
15 69620060
15 50277132
15 46940659
15 48124788
15 6975960
15 49784606
15 5230888
15 9245492
15 47146365
15 8550559
15 46752832
15 10803620
15 26778566
15 9807622
15 7967115
15 34701735
15 9450038
15 35894507
15 25550811
15 20412370
15 15453554
15 63973331
15 10353346
15 28483859
15 10866225
15 35192510
15 28744582
15 6848336
15 27035109
15 14766457
15 11742256
15 18283807
15 47842001
15 51497811
15 6175680
15 46296146
15 45765626
15 17818633
15 7354687
15 22305036
15 7068007
15 22018228
15 46273695
15 11013763
15 22851882
15 8789891
15 24731724
15 17225407
15 28790984
15 20481786
15 31648078
15 11589263
15 44927425
15 9296100
15 18573047
15 47026210
15 16411879
15 16121548
15 7415459
15 19377000
15 9886414
};
\addplot [blue, dashed]
table {%
3 47194067
4 47718402
5 47117642
6 47629805
7 48014968.77
8 48195499
9 48650924
10 52244703
11 61894339
12 63936020
13 66729021
14 72234955
15 73174688
16 78568612
17 85852335
18 89583957
19 94129442
20 96788823
21 73616862
22 0
23 94274171
24 0
25 111964336
};
\addplot [blue]
table {%
3 0
4 0
5 0
6 0
7 47462326.75
8 47443525.3
9 48733935.51
10 52369697.4
11 58433426.1600001
12 65263291.6
13 70483989.03
14 73730412.4
15 79244114.46
16 0
17 0
18 0
19 0
20 0
21 0
22 0
23 0
24 0
25 0
};
\end{axis}

\end{tikzpicture}

==> include/plot_exp1_resampling_subsample50000.tex <==
% This file was created by matplotlib2tikz v0.5.4.
% The lastest updates can be retrieved from
% 
% https://github.com/nschloe/matplotlib2tikz
% 
% where you can also submit bug reports and leavecomments.
% 
\begin{tikzpicture}

\begin{axis}[
xmin=7, xmax=15,
ymin=0, ymax=120000000,
axis on top,
width=\figurewidth,
height=\figureheight
]
\addplot [white!66.666666666666657!black, mark=x, mark size=3, only marks]
table {%
7 6966485
7 10980558
8 20484704
9 19754874
10 20650367
10 31671899
11 23534590
12 22569073
13 24786340
13 24404565
14 66245603
15 50277132
};
\addplot [blue, dashed]
table {%
3 47194067
4 47718402
5 47117642
6 47629805
7 48014968.77
8 48195499
9 48650924
10 52244703
11 61894339
12 63936020
13 66729021
14 72234955
15 73174688
16 78568612
17 85852335
18 89583957
19 94129442
20 96788823
21 73616862
22 0
23 94274171
24 0
25 111964336
};
\addplot [blue]
table {%
3 0
4 0
5 0
6 0
7 47462326.75
8 47443525.3
9 48733935.51
10 52369697.4
11 58433426.1600001
12 65263291.6
13 70483989.03
14 73730412.4
15 79244114.46
16 0
17 0
18 0
19 0
20 0
21 0
22 0
23 0
24 0
25 0
};
\end{axis}

\end{tikzpicture}
